Multimodal analysis of the predictability of hand-gesture properties

Embodied conversational agents benefit from being able to accompany their speech with gestures. Although many data-driven approaches to gesture generation have been proposed in recent years, it is still unclear whether such systems can consistently generate gestures that convey meaning. We investigate which gesture properties (phase, category, and semantics) can be predicted from speech text and/or audio using contemporary deep learning. In extensive experiments, we show that gesture properties related to gesture meaning (semantics and category) are predictable from text features (time-aligned FastText embeddings) alone, but not from prosodic audio features, while rhythm-related gesture properties (phase) on the other hand can be predicted from audio features better than from text. These results are encouraging as they indicate that it is possible to equip an embodied agent with content-wise meaningful co-speech gestures using a machine-learning model.

==> ForCameraReady/ToEdit.tex <==
- Add info about comparisons with the spectrogram

-  one additional condition "TextNoTiming", just to see how much impact the timing information has.

- model that can be trained on a specific speaker, does it then do a better job of predicting for that speaker when compared to the source data for the speaker?  You would need to change the comparison to only use the speakers data for it to be meaningful.  You could then average these scores across speakers.  It could be interesting to look at the individual scores as well to see if some speakers were modeled better than others

- Re-run the WithinSpeak_ID experiments with a one-hot (instead of numerical) speaker encoding

- Add related work about Gesture presence/absence prediction

- report AreaUnderCurve for Speech2GestExist

- report on specific huper-parametesr

- comparing training vs test performance

- Clean up the references section

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typset multiple affiliations (Christoph Sommer)

==> for_the_future_paper/2.related_work.tex <==
\section{Related Work}
Recently field of gesture generation have seen a shift from rule-based \cite{cassell2001beat, lee2006nonverbal, bergmann2009GNetIc} to data-driven \cite{kucherenko2019analyzing, yoon2020speech, ahuja2019react} approaches. We continue this line of research and hence limit this section to the data-driven approaches only.

Previous data-driven approach for gesture generation can be divided in two ways: based on the output data (continous motion vs discrete gesture classes) and based on the input data (audio, text, both or extra info).

\subsection{Discrete gesture generation models}


\subsubsection{Based on audio signal only} \\

\cite{levine2010gesture, chiu2011train, sadoughi2017speech}

\subsubsection{Based on text transcription only}

\cite{neff2008gesture, ishii2018generating}

\subsubsection{Based on both audio and text}

\cite{chiu2015predicting}

\subsubsection{Using not only speech}

\cite{bozkurt2020affective} used both audio prosody and affective state label to generate discrete gesture classes using Hidden Markov Model.

%%%%%%%%%%%   Continuous       ###################

\subsection{Continuous gesture generation models}


\subsubsection{Based on audio signal only} \\


\cite{hasegawa2018evaluation, ferstl2020adversarial, alexanderson2020style, kucherenko2021moving}

\subsubsection{Based on text transcription only}

\cite{yoon2018robots}

\subsubsection{Based on both audio and text}

\cite{kucherenko2020gesticulator, yoon2020speech, ahuja2020no}

And very different approach and problem formulation was used by \cite{yang2020statistics}.

\subsubsection{Using not only speech}

\cite{ahuja2019react}


==> for_the_future_paper/3model.tex <==
\section{Model}

Our model is probabilistic, since the character of human gesticulation is probabilistic: we gesticulate every time differently for exactly the same speech.

There are three main classes of deep probabilistic models:  VAE \cite{kingma2013auto} , GAN \cite{goodfellow2014generative},and Normalizing Flows \cite{rezende2015variational}.

We base our model on the normalizing flows since it provides two key benefits: 1) they produce sharp samples unlike VAEs; 2) they are stable to train and don't have mode-colapse issue unlike GANs.

The most similar model to ours from the previously existing one is FlowWaveNet \cite{kim2018flowavenet}.

==> sec/6limitations.tex <==
\section{Limitations}
The finding presented in Section \ref{sec:experiments} should be taken with caution since the present study has a few limitations we outline below. 

First of all, all the results are established at one direction-giving dataset and might or might not generalise beyond it. We cannot say if the findings are particular to the German language or would generalise to other languages as well. We do not know if the findings are particular to the direction-giving setup or would generalise to other settings. Further experiments on other datasets would help to clarify this uncertainty. %We cannot say if the finding would generalise to another direction-giving dataset in German neither, even though the dataset used is quite large and should be representative.

Secondly, the problem formulation is uncompromising concerning the timing: if the prediction is shifted one frame into the future - it would be counted as wrong. At the same time, we know that people are not very sensitive to small changes in gesture timings \cite{nirme2019motion}. Using a metric that is agnostic to small shifts in time would solve this issue.

%Lastly, the presented system first predicts if the gesture is needed and then predicts gesture properties.  % not fully sure if it is a limitation though

==> tables/OLD_TABLES.tex <==
\footnotesize
\begin{table}
    \centering
    \begin{tabular}{@{}llllll@{}}
        \toprule
         & AlwaysZero & AlwaysOne & UniformRand & InformRand  & Model \\ \midrule
        Accuracy & 85\% $\pm$ 10\% & 15\% $\pm$ 10\% & 50\% $\pm$ 3\% & 76\% $\pm$ 8\% & 85\% $\pm$ 9\% \\ 
        Precision & 0\% $\pm$ 0\% & 15\% $\pm$ 10\% & 15\% $\pm$ 10\% & 17\% $\pm$ 11\% & 51\% $\pm$ 18\% \\ 
        Recall & 0\% $\pm$ 0\% & 100\% $\pm$ 0\% & 51\% $\pm$ 4\% & 14\% $\pm$ 3\% & 39\% $\pm$ 17\% \\ \midrule
        $\text{F}_1$ score for 1 & 0\% $\pm$ 0\% & 25\% $\pm$ 14\% & 21\% $\pm$ 11\% & 14\% $\pm$ 5\% & 41\% $\pm$ 14\% \\ 
        $\text{F}_1$ score for 0  & 92\% $\pm$ 6\% & 0\% $\pm$ 0\% & 62 \% $\pm$ 6\% & 86\% $\pm$ 2\% & 89\% $\pm$ 4\% \\ 
        Macro $\text{F}_1$ score & 46\% $\pm$ 3\% & 13\% $\pm$ 7\% & 42\% $\pm$ 4\% & 50\% $\pm$ 3\% & 65\% $\pm$ 6\% \\ 
        \bottomrule
    \end{tabular}
    \caption{Various evaluation metrics for gesture phase prediction for the gesture semantic property ``shape''. Note that, unlike other tables, models are here reported as columns rather than rows.} \label{tab:Detailed_metrics}
\end{table}
\normalsize


\begin{table}
    \centering
    \begin{tabular}{@{}lllll@{}} %{|l|l|l|l|l|}
    \toprule
        Category & deictic & beat & iconic & discourse \\ %\midrule \midrule
        label frequency & 29.05\% & 14.47\% & 72.03\% & 12.78\% \\ %\midrule \midrule
    \midrule
        AlwaysOne & 20\% $\pm$ 6\% & 13\% $\pm$ 5\% & 43\% $\pm$ 2\% & 11\% $\pm$ \hphantom{0}3\% \\ % \midrule
        AlwaysZero & 43\% $\pm$ 3\% & 46\% $\pm$ 2\% & 20\% $\pm$ 5\% & 46\% $\pm$ 11\% \\ % \midrule
        UniformRandom & 47\% $\pm$ 5\% & 42\% $\pm$ 3\% & 46\% $\pm$ 2\% & 42\% $\pm$ \hphantom{0}2\% \\ % \midrule
        InformedRandom & 50\% $\pm$ 2\% & 50\% $\pm$ 2\% & 50\% $\pm$ 1.5\% & 50\% $\pm$ \hphantom{0}2\% \\ \midrule % \midrule
        AudioOnly & 50\% $\pm$ 3\% & 46\% $\pm$ 2\% & 53\% $\pm$ 5\% & 50\% $\pm$ \hphantom{0}2\% \\ % \midrule
        TextOnly & \textbf{60}\% $\pm$ 6\% & 54\% $\pm$ 3\% & \textbf{64}\% $\pm$ 7\% & \textbf{58}\% $\pm$ \hphantom{0}8\% \\ % \midrule
        BothModalities & \textbf{60}\% $\pm$ 6\% & 53\% $\pm$ 6\% & \textbf{63}\% $\pm$ 5\% & \textbf{59}\% $\pm$ \hphantom{0}7\% \\ % \midrule
    \bottomrule
    \end{tabular}
    \caption{Macro $\text{F}_1$ scores for gesture-category prediction from various speech modalities. In this and following tables, numbers notably above chance performance use bold font.}
    \label{tab:SpModPhrase}
    \vspace{-3mm}
\end{table}

\begin{table}
    \centering
    \begin{tabular}{@{}lllll@{}}
    \toprule
        Semantics & amount & shape & direction & size \\
        Label frequency & 4.7\% & 13.1\% & 13.7\% & 1.9\% \\  \midrule
        AlwaysOne & 4\% $\pm$ 3\% & 13\% $\pm$ 7\% & 10\% $\pm$ 4\% & 3\% $\pm$ 2\% \\ 
        AlwaysZero & 49\% $\pm$ 7\% & 46\% $\pm$ 3\% & 47\% $\pm$ 1.5\% & 49\% $\pm$ 0.6\% \\ 
        UniformRandom & 37\% $\pm$ 2\% & 42\% $\pm$ 4\% & 41\% $\pm$ 3\% & 36\% $\pm$ 2\% \\ 
        InformedRandom & 49\% $\pm$ 1\% & 49\% $\pm$ 2\% & 49\% $\pm$ 2\% & 50\% $\pm$ 1\% \\ \midrule 
        AudioOnly & 49\% $\pm$ 2\% & 49\% $\pm$ 4\% & 50\% $\pm$ 2\% & 49\% $\pm$ 1\% \\
        TextOnly & \textbf{62}\% $\pm$ 11\% & \textbf{65}\% $\pm$ 8\% & \textbf{60}\% $\pm$ 7\% & 57\% $\pm$ 9\% \\
        FullModel & \textbf{63}\% $\pm$ 8\% & \textbf{65}\% $\pm$ 6\% & \textbf{62}\% $\pm$ 8\% & \textbf{59}\% $\pm$ 9\% \\
        \bottomrule
    \end{tabular}
    \caption{Macro $\text{F}_1$ scores for gesture semantics prediction from various speech modalities.}
    \label{tab:SpModSemant}
    \vspace{-3mm}
\end{table}

\footnotesize
\begin{table}
    \centering
    \begin{tabular}{@{}llllll@{}}
    \toprule
        Phase & pre.hold & post hold & stroke & retr & prep \\ \midrule 
        UniformRand & 1.5\% $\pm$ 2\% & 14\% $\pm$ 4\% & 23\% $\pm$ 3\% & 14\% $\pm$ 5\% & 20\% $\pm$ 3\% \\ 
        InformedRand & 1.3\% $\pm$ 4\% & 12\% $\pm$ 4\% & 42\% $\pm$ 4\% & 14\% $\pm$ 5\% & 30\% $\pm$ 3\% \\ \midrule
        AudioOnly & 0\% & 5\% $\pm$ 3\% & \textbf{53}\% $\pm$ 8\% & 12\% $\pm$ 5\% & \textbf{40}\% $\pm$ 4\% \\ 
        TextOnly & 1\% $\pm$ 2\% & 21\% $\pm$ 12\% & \textbf{51}\% $\pm$ 12\% & 25\% $\pm$ 9\% & \textbf{42}\% $\pm$ 7\% \\ 
        FullModel & 0.5\% $\pm$ 1.3\% & 23\% $\pm$ 12\% & \textbf{47}\% $\pm$ 10\% & 25\% $\pm$ 5\% & \textbf{45}\% $\pm$ 6\% \\ 
        \bottomrule
    \end{tabular}
    \caption{Binary $\text{F}_1$ (not Macro $\text{F}_1$) scores for gesture phase prediction from various speech modalities.}
    \label{tab:SpModPhase}
    \vspace{-3mm}
\end{table}

\normalsize



\begin{table}
    \centering
    \begin{tabular}{lllll}
    \toprule
        Category & deictic & beat & iconic & discourse \\ \midrule
        WithSpeakID &59\% $\pm$ 7\% &46\% $\pm$ 2\% &65\% $\pm$ 9\% &61\% $\pm$ 9\% \\
        WithSpeak & 60\% $\pm$ 6\% & 53\% $\pm$ 6\% & 63\% $\pm$ 5\% & 59\% $\pm$ 7\% \\ 
        BetweenSpeak & 57\% $\pm$ 5\% & 49\% $\pm$ 3\% & 55\% $\pm$ 5\% & 56\% $\pm$ 6\% \\ 
        \bottomrule
    \end{tabular}
    \caption{Macro $\text{F}_1$ scores for gesture category prediction within and between the speakers. WithSpeakID indicates using the speaker ID as extra input to the model.}
    \label{tab:GeneralPhrase}
    \vspace{-3mm}
\end{table}


\begin{table}
    \centering
    \begin{tabular}{lllll}
    \toprule
        Semantics & amount & shape & direction & size \\ \midrule
        WithSpeakID &65\% $\pm$ 9\% &64\% $\pm$ 7\% &60\% $\pm$ 8\% &60\% $\pm$ 10\% \\
        WithSpeak & 63\% $\pm$ 8\% & 65\% $\pm$ 6\% & 62\% $\pm$ 8\% & 59\% $\pm$ 9\% \\
        BetweenSpeak & 60\% $\pm$ 7\% & 63\% $\pm$ 8\% & 62\% $\pm$ 7\% & 59\% $\pm$ 12\% \\ 
        \bottomrule
    \end{tabular}
    \caption{Macro $\text{F}_1$ scores for gesture semantics prediction within and between speakers.}
    \label{tab:GeneralSemant}
    \vspace{-3mm}
\end{table}


\footnotesize
\begin{table}
    \centering
    \begin{tabular}{llllll}
    \toprule
        Phase & pre.hold & post hold & stroke & rest & prep \\ \midrule
        WithSpeakID &0\% $\pm$ 0\% &17\% $\pm$ 11\% &56\% $\pm$ 10\% & 17\% $\pm$ 7\% &41\% $\pm$ 6\% \\
        WithSpeak & 0.5\% $\pm$ 1.3\% & 23\% $\pm$ 12\% & 47\% $\pm$ 10\% & 25\% $\pm$ 5\% & 45\% $\pm$ 6\% \\ 
        BetweenSpeak & 1\% $\pm$ 1.5\% & 14\% $\pm$ 8\% & 35\% $\pm$ 8\% & 25\% $\pm$ 8\% & 43\% $\pm$ 6\% \\
        \bottomrule
    \end{tabular}
    \caption{Binary $\text{F}_1$ scores for gesture phase prediction within and between speakers.}
    \label{tab:GeneralPhase}
    \vspace{-3mm}
\end{table}

\normalsize

==> tables/generalisation_ICMI.tex <==
\begin{table*}[t]
\centering
%\rowcolors{3}{}{lightgray} % Coloured rows
% Fit the whole page
\resizebox{\textwidth}{!}{
% Taller lines
\renewcommand{\arraystretch}{1.5}
% Magic for aligning on plus-minus symbol, see property_prediction.text
\begin{tabular}{@{\kern\tabcolsep}r *{39}{r@{\hspace{\tabcolsep}}c@{\hspace{\tabcolsep}}l}@{\kern\tabcolsep}}

\specialrule{\heavyrulewidth}{0pt}{0pt}&
\multicolumn{12}{c}{\textbf{gesture category} [Macro $\text{F}_1$]} & \multicolumn{12}{c}{\textbf{gesture semantics} [Macro $\text{F}_1$]} & \multicolumn{15}{c}{\textbf{gesture phase} [$\text{F}_1$]} \\

\cmidrule(lr){2-13}
\cmidrule(lr){14-25}
\cmidrule(lr){26-40}

label & \multicolumn{3}{c}{deictic} & \multicolumn{3}{c}{beat} & \multicolumn{3}{c}{iconic} & \multicolumn{3}{c}{discourse} & \multicolumn{3}{c}{amount} & \multicolumn{3}{c}{shape} & \multicolumn{3}{c}{direction} & \multicolumn{3}{c}{size} & \multicolumn{3}{c}{pre-hold} & \multicolumn{3}{c}{post-hold} & \multicolumn{3}{c}{stroke} & \multicolumn{3}{c}{retr} & \multicolumn{3}{c}{prep} \\

\specialrule{\lightrulewidth}{0pt}{0pt}
BetweenSpeaker  & 57\% & $\pm$ & 5\% & 49\% & $\pm$ & 3\% & 55\% & $\pm$ & 5\% & 56\% & $\pm$ & 6\% & 60\% & $\pm$ & 7\% & 63\% & $\pm$ & 8\% & 62\% & $\pm$ & 7\% & 59\% & $\pm$ & 12\% & 1\% & $\pm$ & 1.5\%   & 14\% & $\pm$ & 8\%  & 35\% & $\pm$ & 8\%  & 25\% & $\pm$ & 8\% & 43\% & $\pm$ & 6\% \\ 

\rowcolor{lightgray}
WithinSpeaker    & 60\% & $\pm$ & 6\% & 53\% & $\pm$ & 6\% & 63\% & $\pm$ & 5\% & 59\% & $\pm$ & 7\% & 63\% & $\pm$ & 8\% & 65\% & $\pm$ & 6\% & 62\% & $\pm$ & 8\% & 59\% & $\pm$ & 9\%   & 0.5\% & $\pm$ & 1.3\% & 23\% & $\pm$ & 12\% & 47\% & $\pm$ & 10\% & 25\% & $\pm$ & 5\% & 45\% & $\pm$ & 6\% \\

$\text{WithinSpeaker}_{\text{ID}}$  & 60\% & $\pm$ & 6\% & 55\% & $\pm$ & 5\% & 63\% & $\pm$ & 7\% & 60\% & $\pm$ & 9\% & 66\% & $\pm$ & 9\% & 66\% & $\pm$ & 7\% & 62\% & $\pm$ & 8\% & 59\% & $\pm$ & 10\% & 0\% & $\pm$ & 0\%     & 21\% & $\pm$ & 10\% & 55\% & $\pm$ & 9\% & 24\% & $\pm$ & 9\% & 42\% & $\pm$ & 5\% \\

\specialrule{\heavyrulewidth}{0pt}{0pt}
\end{tabular}}
\caption{A comparison of prediction results for different cross-validation strategies. For detailed information see \cref{sec:generalization_study}.}
\label{tab:generalisation}
\end{table*}


==> tables/generalisation_compare.tex <==
\begin{table*}[t]
\centering
%\rowcolors{3}{}{lightgray} % Coloured rows
% Fit the whole page
\resizebox{\textwidth}{!}{
% Taller lines
\renewcommand{\arraystretch}{1.5}
% Magic for aligning on plus-minus symbol, see property_prediction.text
\begin{tabular}{@{\kern\tabcolsep}r *{39}{r@{\hspace{\tabcolsep}}c@{\hspace{\tabcolsep}}l}@{\kern\tabcolsep}}

\specialrule{\heavyrulewidth}{0pt}{0pt}&
\multicolumn{12}{c}{\textbf{gesture category} [Macro $\text{F}_1$]} & \multicolumn{12}{c}{\textbf{gesture semantics} [Macro $\text{F}_1$]} & \multicolumn{15}{c}{\textbf{gesture phase} [$\text{F}_1$]} \\

\cmidrule(lr){2-13}
\cmidrule(lr){14-25}
\cmidrule(lr){26-40}

label & \multicolumn{3}{c}{deictic} & \multicolumn{3}{c}{beat} & \multicolumn{3}{c}{iconic} & \multicolumn{3}{c}{discourse} & \multicolumn{3}{c}{amount} & \multicolumn{3}{c}{shape} & \multicolumn{3}{c}{direction} & \multicolumn{3}{c}{size} & \multicolumn{3}{c}{pre-hold} & \multicolumn{3}{c}{post-hold} & \multicolumn{3}{c}{stroke} & \multicolumn{3}{c}{retr} & \multicolumn{3}{c}{prep} \\

\specialrule{\lightrulewidth}{0pt}{0pt}
BetweenSpeaker  & 57\% & $\pm$ & 5\% & 49\% & $\pm$ & 3\% & 55\% & $\pm$ & 5\% & 56\% & $\pm$ & 6\% & 60\% & $\pm$ & 7\% & 63\% & $\pm$ & 8\% & 62\% & $\pm$ & 7\% & 59\% & $\pm$ & 12\% & 1\% & $\pm$ & 1.5\%   & 14\% & $\pm$ & 8\%  & 35\% & $\pm$ & 8\%  & 25\% & $\pm$ & 8\% & 43\% & $\pm$ & 6\% \\ 

\rowcolor{lime}
BetweenSpeaker & 58\% & $\pm$ & 3\% & 49\% & $\pm$ & 2\% & 56\% & $\pm$ & 5\% & 56\% & $\pm$ & 4\% & 61\% & $\pm$ & 5\% & 67\% & $\pm$ & 7\% & 65\% & $\pm$ & 6\% & 59\% & $\pm$ & 11\% & 0\% & $\pm$ & 0\% & 12\% & $\pm$ & 8\% & 42\% & $\pm$ & 7\% & 20\% & $\pm$ & 6\% & 38\% & $\pm$ & 6\% \\

\rowcolor{lightgray}
WithinSpeaker    & 60\% & $\pm$ & 6\% & 53\% & $\pm$ & 6\% & 63\% & $\pm$ & 5\% & 59\% & $\pm$ & 7\% & 63\% & $\pm$ & 8\% & 65\% & $\pm$ & 6\% & 62\% & $\pm$ & 8\% & 59\% & $\pm$ & 9\%   & 0.5\% & $\pm$ & 1.3\% & 23\% & $\pm$ & 12\% & 47\% & $\pm$ & 10\% & 25\% & $\pm$ & 5\% & 45\% & $\pm$ & 6\% \\

\rowcolor{lime}
WithinSpeaker & 59\% & $\pm$ & 3\% & 50\% & $\pm$ & 2\% & 58\% & $\pm$ & 3\% & 58\% & $\pm$ & 4\% & 63\% & $\pm$ & 8\% & 65\% & $\pm$ & 4\% & 64\% & $\pm$ & 5\% & 57\% & $\pm$ & 9\% & 0\% & $\pm$ & 0\% & 14\% & $\pm$ & 5\% & 47\% & $\pm$ & 3\% & 20\% & $\pm$ & 4\% & 40\% & $\pm$ & 3\% \\


$\text{WithinSpeaker}_{\text{ID}}$  & 60\% & $\pm$ & 6\% & 55\% & $\pm$ & 5\% & 63\% & $\pm$ & 7\% & 60\% & $\pm$ & 9\% & 66\% & $\pm$ & 9\% & 66\% & $\pm$ & 7\% & 62\% & $\pm$ & 8\% & 59\% & $\pm$ & 10\% & 0\% & $\pm$ & 0\%     & 21\% & $\pm$ & 10\% & 55\% & $\pm$ & 9\% & 24\% & $\pm$ & 9\% & 42\% & $\pm$ & 5\% \\

\rowcolor{lime}
$\text{WithinSpeaker}_{\text{ID}}$ & 60\% & $\pm$ & 2\% & 53\% & $\pm$ & 3\% & 62\% & $\pm$ & 4\% & 61\% & $\pm$ & 3\% & 64\% & $\pm$ & 9\% & 67\% & $\pm$ & 7\% & 64\% & $\pm$ & 5\% & 54\% & $\pm$ & 7\% & 0\% & $\pm$ & 0\% & 12\% & $\pm$ & 5\% & 54\% & $\pm$ & 5\% & 22\% & $\pm$ & 7\% & 45\% & $\pm$ & 3\% \\

\specialrule{\heavyrulewidth}{0pt}{0pt}
\end{tabular}}
\caption{A comparison of prediction results for different cross-validation strategies. For detailed information see \cref{sec:generalization_study}.}
\label{tab:generalisation}
\end{table*}


==> tables/property_prediction_IVA.tex <==
% Make the table fit the whole page
\resizebox{\textwidth}{!}{
% Taller lines
\renewcommand{\arraystretch}{1.5}

%One right-aligned column followed by 13*3=39 columns (e.g. deictic is 3 columns because I align on the plus-minus by putting it into a separate middle column). The column triplets are right-center-left aligned.
\begin{tabular}{@{\kern\tabcolsep}r *{39}{r@{\hspace{\tabcolsep}}c@{\hspace{\tabcolsep}}l}@{\kern\tabcolsep}}

\toprule
& \multicolumn{12}{c}{\textbf{gesture category} [Macro $\text{F}_1$]} & \multicolumn{12}{c}{\textbf{gesture semantics} [Macro $\text{F}_1$]} & \multicolumn{15}{c}{\textbf{gesture phase} [$\text{F}_1$]} \\

\cmidrule(lr){2-13}
\cmidrule(lr){14-25}
\cmidrule(lr){26-40}

label & \multicolumn{3}{c}{deictic} & \multicolumn{3}{c}{beat} & \multicolumn{3}{c}{iconic} & \multicolumn{3}{c}{discourse} & \multicolumn{3}{c}{amount} & \multicolumn{3}{c}{shape} & \multicolumn{3}{c}{direction} & \multicolumn{3}{c}{size} & \multicolumn{3}{c}{pre-hold} & \multicolumn{3}{c}{post-hold} & \multicolumn{3}{c}{stroke} & \multicolumn{3}{c}{retr} & \multicolumn{3}{c}{prep} \\

relative frequency & \multicolumn{3}{c}{29.05\%} & \multicolumn{3}{c}{14.47\%} & \multicolumn{3}{c}{72.03\%} & \multicolumn{3}{c}{12.78\%} & \multicolumn{3}{c}{4.7\%} & \multicolumn{3}{c}{13.1\%} & \multicolumn{3}{c}{13.7\%} & \multicolumn{3}{c}{1.9\%} & \multicolumn{3}{c}{0.6\%} & \multicolumn{3}{c}{12.2\%} & \multicolumn{3}{c}{40.9\%} & \multicolumn{3}{c}{14.8\%} & \multicolumn{3}{c}{30.8\%} \\ 

\specialrule{\lightrulewidth}{0pt}{0pt}

\textit{AlwaysOne} & 20\% & $\pm$ & 6\% & 13\% & $\pm$ & 5\% & 43\% & $\pm$ & 2\% & 11\% & $\pm$ & \hphantom{0}3\% & 4\% & $\pm$ & 3\% & 13\% & $\pm$ & 7\% & 10\% & $\pm$ & 4\% & 3\% & $\pm$ & 2\% & & -- & & & -- & & & -- & & & -- & & & -- &          \\

\rowcolor{lightgray}
\textit{AlwaysZero} & 43\% & $\pm$ & 3\%  & 46\% & $\pm$ & 2\% & 20\% & $\pm$ & 5\%  & 46\% & $\pm$ & 11\%  & 49\% & $\pm$ & 7\%   & 46\% & $\pm$ & \hphantom{0}3\%  & 47\% & $\pm$ & 1.5\%        & 49\% & $\pm$ & 0.6\%        & & -- &    & & -- &  & & -- &   & & -- && & -- &          \\

\textit{UniformRandom}   & 47\% & $\pm$ & 5\%  & 42\% & $\pm$ & 3\% & 46\% & $\pm$ & 2\%  & 42\% & $\pm$ & \hphantom{0}2\%  & 37\% & $\pm$ & 2\%   & 42\% & $\pm$ & 4\%  & 41\% & $\pm$ & 3\%  & 36\% & $\pm$ & 2\%  & 1.5\% & $\pm$ & 2\%   & 14\% & $\pm$ & 4\%  & 23\% & $\pm$ & 3\%   & 14\% & $\pm$ & 5\% & 20\% & $\pm$ & 3\%          \\

\rowcolor{lightgray}
\textit{InformedRandom}  & 50\% & $\pm$ & 2\%  & 50\% & $\pm$ & 2\% & 50\% & $\pm$ & 1.5\%        & 50\% & $\pm$ & \hphantom{0}2\%  & 49\% & $\pm$ & 1\%   & 49\% & $\pm$ & 2\%  & 49\% & $\pm$ & 2\%  & 50\% & $\pm$ & 1\%  & 1.3\% & $\pm$ & 4\%   & 12\% & $\pm$ & 4\%  & 42\% & $\pm$ & 4\%   & 14\% & $\pm$ & 5\% & 30\% & $\pm$ & 3\%          \\ 

\specialrule{\lightrulewidth}{0pt}{0pt}
\rowcolor{white}
AudioOnly       & 50\% & $\pm$ & 3\%  & 46\% & $\pm$ & 2\% & 53\% & $\pm$ & 5\%  & 50\% & $\pm$ & \hphantom{0}2\%  & 49\% & $\pm$ & 2\%   & 49\% & $\pm$ & 4\%  & 50\% & $\pm$ & 2\%  & 49\% & $\pm$ & 1\%  & & 0\% &    & 5\% & $\pm$ & 3\%   & \highlight{53\%} & \highlight{$\pm$} & \highlight{8\%}  & 12\% & $\pm$ & 5\% & \highlight{40\%} & \highlight{$\pm$} & \highlight{4\%} \\

\rowcolor{lightgray}

TextWithTiming        & \highlight{60\%} & \highlight{$\pm$} & \highlight{6\%} & 54\% & $\pm$ & 3\% & \highlight{64\%} & \highlight{$\pm$} & \highlight{7\%} & \highlight{58\%} & \highlight{$\pm$} & \highlight{\hphantom{0}8\%} & \highlight{62\%} & \highlight{$\pm$} & \highlight{11\%} & \highlight{65\%} & \highlight{$\pm$} & \highlight{8\%} & \highlight{60\%} & \highlight{$\pm$} & \highlight{7\%} & 57\% & $\pm$ & 9\%  & 1\% & $\pm$ & 2\%     & 21\% & $\pm$ & 12\% & \highlight{51\%} & \highlight{$\pm$} & \highlight{12\%} & 25\% & $\pm$ & 9\% & \highlight{42\%} & \highlight{$\pm$} & \highlight{7\%} \\

\rowcolor{white}

TextNoTiming        & \highlight{61\%} & \highlight{$\pm$} & \highlight{6\%} & 56\% & $\pm$ & 5\% & \highlight{63\%} & \highlight{$\pm$} & \highlight{7\%} & \highlight{60\%} & \highlight{$\pm$} & \highlight{\hphantom{0}8\%} & \highlight{68\%} & \highlight{$\pm$} & \highlight{8\%} & \highlight{66\%} & \highlight{$\pm$} & \highlight{7\%} & \highlight{61\%} & \highlight{$\pm$} & \highlight{9\%} & 59\% & $\pm$ & 12\%  & 0\% & $\pm$ & 0\%     & 18\% & $\pm$ & 11\% & \highlight{54\%} & \highlight{$\pm$} & \highlight{11\%} & 19\% & $\pm$ & 7\% & \highlight{39\%} & \highlight{$\pm$} & \highlight{7\%} \\

\rowcolor{lightgray}

BothModalities  & \highlight{60\%} & \highlight{$\pm$} & \highlight{6\%} & 53\% & $\pm$ & 6\% & \highlight{63\%} & \highlight{$\pm$} & \highlight{5\%} & \highlight{59\%} & \highlight{$\pm$} & \highlight{\hphantom{0}7\%} & \highlight{63\%} & \highlight{$\pm$} & \highlight{8\%}  & \highlight{65\%} & \highlight{$\pm$} & \highlight{6\%} & \highlight{62\%} & \highlight{$\pm$} & \highlight{8\%} & \highlight{59\%} & \highlight{$\pm$} & \highlight{9\%} & 0.5\% & $\pm$ & 1.3\% & 23\% & $\pm$ & 12\% & \highlight{47\%} & \highlight{${\pm}$} & \highlight{10\%} & 25\% & $\pm$ & 5\% & \highlight{45\%} & \highlight{$\pm$} & \highlight{6\%} \\ 

\bottomrule
\end{tabular}}

==> tables/property_prediction_compare.tex <==
% Make the table fit the whole page
\resizebox{\textwidth}{!}{
% Taller lines
\renewcommand{\arraystretch}{1.5}

%One right-aligned column followed by 13*3=39 columns (e.g. deictic is 3 columns because I align on the plus-minus by putting it into a separate middle column). The column triplets are right-center-left aligned.
\begin{tabular}{@{\kern\tabcolsep}r *{39}{r@{\hspace{\tabcolsep}}c@{\hspace{\tabcolsep}}l}@{\kern\tabcolsep}}

\toprule
& \multicolumn{12}{c}{\textbf{gesture category} [Macro $\text{F}_1$]} & \multicolumn{12}{c}{\textbf{gesture semantics} [Macro $\text{F}_1$]} & \multicolumn{15}{c}{\textbf{gesture phase} [$\text{F}_1$]} \\

\cmidrule(lr){2-13}
\cmidrule(lr){14-25}
\cmidrule(lr){26-40}

label & \multicolumn{3}{c}{deictic} & \multicolumn{3}{c}{beat} & \multicolumn{3}{c}{iconic} & \multicolumn{3}{c}{discourse} & \multicolumn{3}{c}{amount} & \multicolumn{3}{c}{shape} & \multicolumn{3}{c}{direction} & \multicolumn{3}{c}{size} & \multicolumn{3}{c}{pre-hold} & \multicolumn{3}{c}{post-hold} & \multicolumn{3}{c}{stroke} & \multicolumn{3}{c}{retr} & \multicolumn{3}{c}{prep} \\

relative frequency & \multicolumn{3}{c}{29.05\%} & \multicolumn{3}{c}{14.47\%} & \multicolumn{3}{c}{72.03\%} & \multicolumn{3}{c}{12.78\%} & \multicolumn{3}{c}{4.7\%} & \multicolumn{3}{c}{13.1\%} & \multicolumn{3}{c}{13.7\%} & \multicolumn{3}{c}{1.9\%} & \multicolumn{3}{c}{0.6\%} & \multicolumn{3}{c}{12.2\%} & \multicolumn{3}{c}{40.9\%} & \multicolumn{3}{c}{14.8\%} & \multicolumn{3}{c}{30.8\%} \\ 

\specialrule{\lightrulewidth}{0pt}{0pt}

\textit{AlwaysOne} & 20\% & $\pm$ & 6\% & 13\% & $\pm$ & 5\% & 43\% & $\pm$ & 2\% & 11\% & $\pm$ & \hphantom{0}3\% & 4\% & $\pm$ & 3\% & 13\% & $\pm$ & 7\% & 10\% & $\pm$ & 4\% & 3\% & $\pm$ & 2\% & & -- & & & -- & & & -- & & & -- & & & -- &          \\

\rowcolor{lime}
\textit{AlwaysOne} & 23\% & $\pm$ & 3\% & 14\% & $\pm$ & 3\% & 41\% & $\pm$ & 2\% & 12\% & $\pm$ & 2\% & 5\% & $\pm$ & 2\% & 11\% & $\pm$ & 4\% & 12\% & $\pm$ & 4\% & 2\% & $\pm$ & 1\% & & -- & & & -- & & & -- & & & -- & & & -- &          \\


\rowcolor{lightgray}
\textit{AlwaysZero} & 43\% & $\pm$ & 3\%  & 46\% & $\pm$ & 2\% & 20\% & $\pm$ & 5\%  & 46\% & $\pm$ & 11\%  & 49\% & $\pm$ & 7\%   & 46\% & $\pm$ & \hphantom{0}3\%  & 47\% & $\pm$ & 1.5\%        & 49\% & $\pm$ & 0.6\%        & & -- &    & & -- &  & & -- &   & & -- && & -- &          \\

\rowcolor{lime}
\textit{AlwaysZero} & 41\% & $\pm$ & 2\% & 46\% & $\pm$ & 1\% & 23\% & $\pm$ & 3\% & 46\% & $\pm$ & 1\% & 49\% & $\pm$ & 1\% & 47\% & $\pm$ & 1\% & 46\% & $\pm$ & 1\% & 49\% & $\pm$ & 1\% & & -- & & & -- & & & -- & & & -- & & & -- &          \\


\textit{UniformRandom}   & 47\% & $\pm$ & 5\%  & 42\% & $\pm$ & 3\% & 46\% & $\pm$ & 2\%  & 42\% & $\pm$ & \hphantom{0}2\%  & 37\% & $\pm$ & 2\%   & 42\% & $\pm$ & 4\%  & 41\% & $\pm$ & 3\%  & 36\% & $\pm$ & 2\%  & 1.5\% & $\pm$ & 2\%   & 14\% & $\pm$ & 4\%  & 23\% & $\pm$ & 3\%   & 14\% & $\pm$ & 5\% & 20\% & $\pm$ & 3\%          \\

\rowcolor{lime}
\textit{UniformRandom} & 48\% & $\pm$ & 1\% & 43\% & $\pm$ & 2\% & 48\% & $\pm$ & 1\% & 42\% & $\pm$ & 1\% & 37\% & $\pm$ & 2\% & 42\% & $\pm$ & 3\% & 42\% & $\pm$ & 3\% & 35\% & $\pm$ & 1\% & 1.4\% & $\pm$ & 0.8\% & 16\% & $\pm$ & 3\% & 36\% & $\pm$ & 16\% & 18\% & $\pm$ & 4\% & 26\% & $\pm$ & 7\% \\


\rowcolor{lightgray}
\textit{InformedRandom}  & 50\% & $\pm$ & 2\%  & 50\% & $\pm$ & 2\% & 50\% & $\pm$ & 1.5\%        & 50\% & $\pm$ & \hphantom{0}2\%  & 49\% & $\pm$ & 1\%   & 49\% & $\pm$ & 2\%  & 49\% & $\pm$ & 2\%  & 50\% & $\pm$ & 1\%  & 1.3\% & $\pm$ & 4\%   & 12\% & $\pm$ & 4\%  & 42\% & $\pm$ & 4\%   & 14\% & $\pm$ & 5\% & 30\% & $\pm$ & 3\%          \\ 

\rowcolor{lime}
\textit{InformedRandom} & 50\% & $\pm$ & 1\% & 50\% & $\pm$ & 1\% & 50\% & $\pm$ & 1\% & 50\% & $\pm$ & 1\% & 50\% & $\pm$ & 1\% & 50\% & $\pm$ & 1\% & 50\% & $\pm$ & 1\% & 50\% & $\pm$ & 1\% & 1\% & $\pm$ & 1.4\% & 14\% & $\pm$ & 3\% & 46\% & $\pm$ & 10\% & 16\% & $\pm$ & 4\% & 32\% & $\pm$ & 5\% \\

\specialrule{\lightrulewidth}{0pt}{0pt}
\rowcolor{white}
AudioOnly       & 50\% & $\pm$ & 3\%  & 46\% & $\pm$ & 2\% & 53\% & $\pm$ & 5\%  & 50\% & $\pm$ & \hphantom{0}2\%  & 49\% & $\pm$ & 2\%   & 49\% & $\pm$ & 4\%  & 50\% & $\pm$ & 2\%  & 49\% & $\pm$ & 1\%  & & 0\% &    & 5\% & $\pm$ & 3\%   & \highlight{53\%} & \highlight{$\pm$} & \highlight{8\%}  & 12\% & $\pm$ & 5\% & \highlight{40\%} & \highlight{$\pm$} & \highlight{4\%} \\

\rowcolor{lime}
AudioOnly & 52\% & $\pm$ & 1\% & 51\% & $\pm$ & 2\% & 53\% & $\pm$ & 3\% & 52\% & $\pm$ & 2\% & 50\% & $\pm$ & 1\% & 51\% & $\pm$ & 1\% & 51\% & $\pm$ & 2\% & 50\% & $\pm$ & 1\% & 0\% & $\pm$ & 0\% & 7\% & $\pm$ & 3\% & 53\% & $\pm$ & 4\% & 15\% & $\pm$ & 4\% & 41\% & $\pm$ & 3\% \\


\rowcolor{lightgray}

TextWithTiming        & \highlight{60\%} & \highlight{$\pm$} & \highlight{6\%} & 54\% & $\pm$ & 3\% & \highlight{64\%} & \highlight{$\pm$} & \highlight{7\%} & \highlight{58\%} & \highlight{$\pm$} & \highlight{\hphantom{0}8\%} & \highlight{62\%} & \highlight{$\pm$} & \highlight{11\%} & \highlight{65\%} & \highlight{$\pm$} & \highlight{8\%} & \highlight{60\%} & \highlight{$\pm$} & \highlight{7\%} & 57\% & $\pm$ & 9\%  & 1\% & $\pm$ & 2\%     & 21\% & $\pm$ & 12\% & \highlight{51\%} & \highlight{$\pm$} & \highlight{12\%} & 25\% & $\pm$ & 9\% & \highlight{42\%} & \highlight{$\pm$} & \highlight{7\%} \\

\rowcolor{lime}
TextWithTiming & 59\% & $\pm$ & 3\% & 50\% & $\pm$ & 2\% & 60\% & $\pm$ & 4\% & 59\% & $\pm$ & 5\% & 64\% & $\pm$ & 9\% & 67\% & $\pm$ & 5\% & 65\% & $\pm$ & 4\% & 56\% & $\pm$ & 8\% & 0\% & $\pm$ & 0\% & 14\% & $\pm$ & 4\% & 47\% & $\pm$ & 3\% & 21\% & $\pm$ & 4\% & 41\% & $\pm$ & 4\% \\


\rowcolor{white}

TextNoTiming        & \highlight{61\%} & \highlight{$\pm$} & \highlight{6\%} & 56\% & $\pm$ & 5\% & \highlight{63\%} & \highlight{$\pm$} & \highlight{7\%} & \highlight{60\%} & \highlight{$\pm$} & \highlight{\hphantom{0}8\%} & \highlight{68\%} & \highlight{$\pm$} & \highlight{8\%} & \highlight{66\%} & \highlight{$\pm$} & \highlight{7\%} & \highlight{61\%} & \highlight{$\pm$} & \highlight{9\%} & 59\% & $\pm$ & 12\%  & 0\% & $\pm$ & 0\%     & 18\% & $\pm$ & 11\% & \highlight{54\%} & \highlight{$\pm$} & \highlight{11\%} & 19\% & $\pm$ & 7\% & \highlight{39\%} & \highlight{$\pm$} & \highlight{7\%} \\

\rowcolor{lightgray}

BothModalities  & \highlight{60\%} & \highlight{$\pm$} & \highlight{6\%} & 53\% & $\pm$ & 6\% & \highlight{63\%} & \highlight{$\pm$} & \highlight{5\%} & \highlight{59\%} & \highlight{$\pm$} & \highlight{\hphantom{0}7\%} & \highlight{63\%} & \highlight{$\pm$} & \highlight{8\%}  & \highlight{65\%} & \highlight{$\pm$} & \highlight{6\%} & \highlight{62\%} & \highlight{$\pm$} & \highlight{8\%} & \highlight{59\%} & \highlight{$\pm$} & \highlight{9\%} & 0.5\% & $\pm$ & 1.3\% & 23\% & $\pm$ & 12\% & \highlight{47\%} & \highlight{${\pm}$} & \highlight{10\%} & 25\% & $\pm$ & 5\% & \highlight{45\%} & \highlight{$\pm$} & \highlight{6\%} \\ 

\rowcolor{lime}
BothModalities & 59\% & $\pm$ & 3\% & 50\% & $\pm$ & 2\% & 58\% & $\pm$ & 3\% & 58\% & $\pm$ & 4\% & 63\% & $\pm$ & 8\% & 65\% & $\pm$ & 4\% & 64\% & $\pm$ & 5\% & 57\% & $\pm$ & 9\% & 0\% & $\pm$ & 0\% & 14\% & $\pm$ & 5\% & 47\% & $\pm$ & 3\% & 20\% & $\pm$ & 4\% & 40\% & $\pm$ & 3\% \\
\bottomrule
\end{tabular}}
